KKANs: Kurkova-Kolmogorov-Arnold Networks and Their Learning Dynamics

Inspired by the Kolmogorov-Arnold representation theorem and Kurkova's principle of using approximate representations, we propose the Kurkova-Kolmogorov-Arnold Network (KKAN), a new two-block architecture that combines robust multi-layer perceptron (MLP) based inner functions with flexible linear combinations of basis functions as outer functions. We first prove that KKAN is a universal approximator, and then we demonstrate its versatility across scientific machine-learning applications, including function regression, physics-informed machine learning (PIML), and operator-learning frameworks. The benchmark results show that KKANs outperform MLPs and the original Kolmogorov-Arnold Networks (KANs) in function approximation and operator learning tasks and achieve performance comparable to fully optimized MLPs for PIML. To better understand the behavior of the new representation models, we analyze their geometric complexity and learning dynamics using information bottleneck theory, identifying three universal learning stages, fitting, transition, and diffusion, across all types of architectures. We find a strong correlation between geometric complexity and signal-to-noise ratio (SNR), with optimal generalization achieved during the diffusion stage. Additionally, we propose self-scaled residual-based attention weights to maintain high SNR dynamically, ensuring uniform convergence and prolonged learning.

==> HistoryTable.tex <==
%\section{Appendix}
\begin{table}[H]
    \centering
    \scriptsize
    \begin{tabular}{|p{8cm}|p{4.5cm}|p{0.5cm}|}
    \hline
        Publication & Contribution  & Year \\\hline
         Physics Informed Deep Learning (Part I): Data-driven solutions of nonlinear Partial Differential Equations~\citep{raissi2017physicsI}& PINN framework for solving PDEs & 2017 \\\hline
         Physics Informed Deep Learning (Part II): Data-driven discovery of nonlinear Partial Differential Equations~\citep{raissi2017physicsII}& PINN framework for PDE discovery & 2017 \\\hline
         Hidden Fluid Mechanics: A Navier-Stokes informed deep learning framework for assimilating flow visualization Data~\citep{raissi2018hiddenfluidmechanicsnavierstokes}& Uncovers hidden fields, uses weight normalization & 2018 \\\hline
        fPINNs: Fractional Physics-Informed Neural Networks~ \citep{pang2019fpinns}& Extends PINNs to fractional PDEs & 2018 \\\hline
        Quantifying total uncertainty in physics-informed neural networks for solving forward and inverse stochastic problems \citep{zhang2019quantifying}& Introduces UQ for PINNs & 2018 \\\hline
         Physics-informed neural networks: A deep learning framework for solving forward and inverse problems involving nonlinear partial differential equations~\citep{raissi2019physics}& Journal paper formalizing PINNs & 2019 \\\hline
        Multi-scale Deep Neural Networks for Solving High-Dimensional PDEs~\citep{cai2019multi}& Introduces multi-scale feature expansions & 2019 \\\hline
         Variational Physics-Informed Neural Networks For Solving Partial Differential Equations~\citep{kharazmi2019variationalphysicsinformedneuralnetworks}& Extends PINNs using variational approaches & 2019 \\\hline
         DeepOnet: Learning nonlinear operators for identifying differential equations based on the universal approximation theorem of operators \citep{lu2019deeponet}& Introduces DeepONets & 2019 \\\hline
         DeepXDE: A deep learning library for solving differential equations \citep{lu2021deepxde}& First PIML library and introduction to resampling & 2019 \\\hline
         On the convergence of physics-informed neural networks for linear second-order elliptic and parabolic type PDEs~\citep{shin2020convergence}& Convergence and error bounds for PINNs & 2020 \\\hline
         When and why PINNs fail to train: A neural tangent kernel perspective~\citep{wang2020pinnsfailtrainneural}& NTK analysis for PINN  & 2020 \\\hline
        Extended physics-informed neural networks (XPINNs): A generalized space-time domain decomposition-based deep learning framework for nonlinear partial differential equations~\citep{jagtap2020extended}& Domain decomposition for PINNs & 2020 \\\hline
        Locally adaptive activation functions with slope recovery for deep and physics-informed neural networks \citep{jagtap2020locally}& Introduces adaptive activation functions & 2020 \\\hline
         B-PINNs: Bayesian Physics-Informed Neural Networks for forward and inverse PDE problems with noisy Data \citep{yang2021b}& Bayesian PINNs for noisy data & 2020 \\\hline
         Self-adaptive physics-informed neural networks using a soft attention mechanism~\citep{mcclenny2020self}& Introduces local weights an attention mechanisms & 2020 \\\hline
         On the eigenvector bias of Fourier feature networks: From regression to solving multi-scale PDEs with physics-informed neural networks~\citep{Wang2020_Fourier_nets}& Fourier features for multi-scale PDEs & 2020 \\\hline
         Separable Physics-Informed Neural Networks~\citep{cho2023separablephysicsinformedneuralnetworks}& Speeds up training up to 100 times & 2023 \\\hline
         Artificial to Spiking Neural Networks Conversion for Scientific Machine Learning~\citep{zhang2023artificial}& Extends PIML to Spiking NNs & 2023 \\\hline
         Residual-based attention and connection to information bottleneck theory in PINNs~\citep{anagnostopoulos2023residual}& Connection to information bottleneck theory & 2023 \\\hline
         Stacked networks improve physics-informed training: applications to neural networks and deep operator networks~\citep{howard2023stacked}& Stacked training improves performance & 2023 \\\hline
         Multi-stage Neural Networks: Function approximator of machine precision~\citep{wang2023multistageneuralnetworksfunction}& Multi-stage training for better performance & 2023 \\\hline
         Tackling the curse of dimensionality with Physics-Informed Neural Networks \citep{hu2024tackling}& Solves PDEs with up to 100,000 dimensions & 2023 \\\hline
         KAN: Kolmogorov-Arnold networks~\citep{liu2024kan}& Extension to KANs & 2024 \\\hline
 \end{tabular}
    \caption{Evolution of the algorithmic variants}
    \label{tab:Variants1}
\end{table}


